Data-Driven Structured Robust Control of Linear Systems

Static structured control refers to the task of designing a state-feedback controller such that the control gain satisfies a subspace constraint. Structured control has applications in control of communication-inhibited dynamical systems, such as systems in networked environments. This work performs $H_2$-suboptimal regulation under a common structured state-feedback controller for a class of data-consistent plants. The certification of $H_2$-performance is attained through a combination of standard $H_2$ LMIs, convex sufficient conditions for structured control, and a matrix S-lemma for set-membership. The resulting convex optimization problems are linear matrix inequalities whose size scales independently of the number of data samples collected. Data-driven structured $H_2$-regulation control is demonstrated on example systems.

==> sections/contributions.tex <==
\urg{Contributions of this work are,
\begin{itemize}
    \item Contributions
    \item go
    \item here
\end{itemize}}

==> sections/extensions.tex <==
\section{Extensions}



==> sections/h2_control.tex <==
\section{H2 control}

\label{sec:h2}
\urg{Do we have space to talk about worst-case suboptimal $H_2$ control? Should we instead focus the entire paper around $H_2$ control?}

A discrete-time system with exogenous input $\xi \in \R^{q}$ and input 
